OpenUVR: an Open-Source System Framework for Untethered Virtual Reality Applications

Advancements in heterogeneous computing technologies enable the significant potential of virtual reality (VR) applications. To offer the best user experience (UX), a system should adopt an untethered, wireless-network-based architecture to transfer VR content between the user and the content generator. However, modern wireless network technologies make implementing such an architecture challenging, as VR applications require superior video quality -- with high resolution, high frame rates, and very low latency. This paper presents OpenUVR, an open-source framework that uses commodity hardware components to satisfy the demands of interactive, real-time VR applications. OpenUVR significantly improves UX through a redesign of the system stack and addresses the most time-sensitive issues associated with redundant memory copying in modern computing systems. OpenUVR presents a cross-layered VR datapath to avoid redundant data operations and computation among system components, OpenUVR customizes the network stack to eliminate unnecessary memory operations incurred by mismatching data formats in each layer, and OpenUVR uses feedback from mobile devices to remove memory buffers. Together, these modifications allow OpenUVR to reduce VR application delays to 14.32 ms, meeting the 20 ms minimum latency in avoiding motion sickness. As an open-source system that is fully compatible with commodity hardware, OpenUVR offers the research community an opportunity to develop, investigate, and optimize applications for untethered, high-performance VR architectures.

==> Makefile <==
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))

ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe

PREFIX=c:\\cygwin\\home\\$(USER)\\papers\\2008SASP-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac

ifeq ($(USER),mbt)
ALL = show_nt
ACROREAD = kpdf
else
ALL =  pdf
endif

endif

TEX_STUFF= $(wildcard *.tex)
PDF_TARGETS= paper.pdf
FIGURES = $(wildcard Figures/*.pdf) $(wildcard Graphs/*.pdf)

.PHONY: test_build clean

all: $(ALL)

paper.pdf:  $(FIGURES) Makefile 


test_build:
	rm -rf _test_build
	mkdir _test_build
	(REPO=$$(svn info | grep URL | sed 's/URL: //');\
	 DIR=$$(svn info | grep URL | sed 's/.*\///');\
	 cd _test_build; \
	 svn checkout $$REPO;\
	 cd $$DIR;\
	 make;\
	 open paper.pdf;\
	)	

%_abbrv.bib: %.bib
	./abbrv.py $< $@

pdf: $(PDF_TARGETS)

%.aux : %.tex $(TEX_STUFF)
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	pdftops $*.pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $*.ps
#	cp $*.pdf 122-OX997-Tseng.pdf
#
# copies file to prevent write-after-read problems
# uses date as suffix.
#
show_nt: pdf
	- killall $(ACROREAD)
	cp paper.pdf paper_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)paper_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out $(PDF_TARGETS)
	rm -rf paper_abbrv.bib 
	rm -rf _test_build





==> discussions.tex <==
\section{\CMFdel{Discussion}\CMF{Additional Considerations and Comparisons}}
\label{sec:discussions}
In addition to \CMFdel{the optimizations we made in designing}\CMF{optimizing}
\OpenWVR{}, we \CMFdel{considered other factors in the \OpenWVR{} system
architecture and their potential impact on performance}\CMF{examined
\OpenWVR{}'s performance
using synchronous/asynchronous modes and mmWave wireless technologies}.
We also compare\CMF{d} \CMFdel{our}\CMF{\OpenWVR{}'s}
latency with \CMFdel{a}\CMF{the latencies of two}
state-of-the-art\CMF{,} \CMF{commercial}\CMFdel{ized,
proprietary product that can potentially serve a similar purpose.}
\CMF{gaming systems---Steam Link and GamingAnywhere}.

\ignore{
While our GTX 1070 GPU saw tremendous speedups when copying data within GPU memory
rather than between GPU memory and RAM, we found that not all GPUs will see the same
level of performance boost. We found that our Quadro P4000 was 3.2~ms faster than our
baseline GPU at reading pixel data to RAM, but its encoding was 0.7~ms slower. The GTX
1070 encoding time improved from 9.1~ms down to 3.5~ms when we introduced our CUDA
integration optimization, while the Quadro P4000 improved from 7.3~ms down to 4.5~ms.
The measured visual latency remained about the same on each, with a median lag of 2 frames, which at 90 fps is around 22~ms.
}

\subsection{Synchronous \OpenWVR{}}
In its default configuration, \OpenWVR{} initiates a\CMF{n independent}\CMFdel{ separate} thread
that \CMF{uses a specific GPU-memory location to }continually encode\CMFdel{s}\CMF{ data} and transmit\CMFdel{s} \CMFdel{data}\CMF{it} to the MUD\CMFdel{from a specified
GPU memory location}. This design \CMFdel{allows}\CMF{means that} \OpenWVR{}'s encoding and
communication process\CMF{es} \CMFdel{to}\CMF{can} pipeline with\CMFdel{ the} VR\CMF{-}content generation, improving
the throughput of system resources.

Th\CMFdel{is}\CMF{e default \OpenWVR{}} configuration\CMF{ also} allows the host
to generate content at high framerates (90 FPS \CMFdel{in our case using}\CMF{for}
Quake 3\CMF{ Arena}).
\CMFdel{However, as}\CMF{But} the Raspberry Pi-based MUD can only decode and
display video at 60~FPS,\CMF{ so} generating
VR content at 90~FPS does not \CMFdel{benefit}\CMF{improve UX}\CMFdel{ the VR
user's experience}.
An application that can render at 90~FPS takes at most 1/90th of a second,
or 11.1~ms, to execute its game loop. If \CMFdel{it}\CMF{the application} runs
at 60~FPS instead, it has 16.7~ms to run its game loop, giving it 5.6~ms of
slack\CMFdel{ during which it can}\CMF{ time to} perform \OpenWVR{}'s tasks, which only take around 3.6~ms.

\CMFdel{Therefore, }\OpenWVR{} can \CMF{thus }provide a synchronous API \CMFdel{for the game
to explicitly}\CMF{that a game can use to }trigger \CMFdel{the }encoding and data\CMF{-}exchange
tasks. \CMFdel{This configuration doesn't require}\CMF{The lack of need for}
a separate thread\CMF{ also frees up the CPU}\CMFdel{, which reduces the usage of a
full CPU core}, potentially lowering \CMFdel{the }power consumption \CMF{and/}or
\CMF{the cost}\CMFdel{price} of the host PC. \CMFdel{Throughout}\CMF{In} our experiments,
we did not observe any significant change in visual latency or quality between
these synchronous and async\CMFdel{rh}\CMF{hr}onous modes of operation. \CMFcom{The
information about \OpenWVR{}'s asynchronous mode appears to have been removed; please
restore it in some form so that the above discussion makes more sense.}

\ignore{
On the host PC, \OpenWVR{} can operate optionally in either a synchronous or asynchronous
manner in relation to the host game's rendering rate. If asynchronous mode is chosen, then
the application will initiate a separate thread which will continually encode and send data
from a specified GPU memory location at 60~FPS, regardless of the state of the game itself.
It is the game's responsibility to copy pixel data into that buffer whenever it wants to
update the pixel content that \OpenWVR{} is sending. This is the recommended mode of operation, as it allows the game to render natively at a frame rate greater than 60~FPS, while allowing \OpenWVR{} to encode 60~FPS.

The game can optionally use \OpenWVR{}'s API to send frames synchronously as well. Current technology operating as the MUD is designed to decode H264 frames at no more than 60~FPS, and trying to decode at higher rates causes video frames to queue within the MUD's GPU memory, which greatly increases latency. Therefore, the caller should be careful not to send more than 60 frames each second. This limits the host game to render at 60~FPS if it wishes to synchronize the rendering and transmission of frames.

We measured the visual latency associated with synchronous and asynchronous 60~FPS for the optimized version of \OpenWVR{}. We found that asynchronous sending incurs an average delay of 1.8 frames at 90~FPS, which is a delay of about 20 ms, while synchronous mode has an average delay of 1.2 frames at 60~FPS, which is also about 20~ms.
}

\subsection{Compar\CMFdel{ing}\CMF{isons} with Steam Link}
Though \OpenWVR{} \CMFdel{targets}\CMF{is intended for} VR applications,
\CMFdel{\OpenWVR{}}\CMF{it} can also serve as a platform for remote interactive gaming.
\CMF{To  evaluate \OpenWVR{}'s performance in this arena, we compared it with}
Steam Link~\cite{SteamLink}\CMFdel{ is a
state-of-the-art commercialized solution for that purpose}.
\CMF{Like \OpenWVR{}, }Steam Link\CMFdel{ also}
relies on a host PC to generate \CMFdel{the }game content and
\CMFdel{react to}\CMF{processes} user input through a wirelessly connected\CMFdel{ Steam Link} set-top box\CMFdel{, similar to the
setup of \OpenWVR{}}.

We tested \CMF{\OpenWVR{} }\CMFdel{several}\CMF{and} Steam Link \CMF{using several }games \CMFdel{using}\CMF{and} the same host PC.
\CMFdel{The}\CMF{Steam Link's} average visual
latency\CMFdel{ we measured} for these games was 3.2 frames, with \CMFdel{the}\CMF{a} minim\CMFdel{al}\CMF{um} latency
\CMFdel{at}\CMF{of} 2 frames, \CMF{which is }almost twice the latency of optimized \OpenWVR{}.
\CMFdel{In addition,}\CMF{It's worth noting that even though} Steam Link\CMF{'s}\CMFdel{ makes the} software library\CMF{ is}
public, \CMFdel{but uses proprietary}\CMF{its} hardware components\CMF{ are proprietary}.\CMF{ So} \OpenWVR{}'s open
architecture provides more \CMFdel{flexibility in}\CMF{options for} configuration\CMFdel{s} and\CMFdel{ further}
optimization\CMFdel{s}.

\subsection{Compar\CMFdel{ing}\CMF{isons} with GamingAnywhere}
GamingAnywhere~\cite{GamingAnywhere} is a popular\CMF{,} open-source\CMF{,} cloud\CMF{-based}
game streaming platform. \CMF{GamingAnywhere renders}\CMFdel{The game's}
content\CMFdel{ is rendered} on high-end servers
in the cloud and \CMFdel{is }stream\CMFdel{ed}\CMF{s the content} to low-end PCs
over the internet. We installed the
GamingAnywhere server on our host PC and installed the client on the Raspberry
Pi\CMFdel{, and}\CMF{. We then} tested \CMF{GamingAnywhere's performance }\CMFdel{it
over}\CMF{using} the same wireless connection\CMFdel{ as}\CMF{, hardware, and network
configuration that we used }with \OpenWVR{}.\CMFdel{ With
the same hardware and network configuration,} GamingAnywhere \CMFdel{can}\CMF{could} only render
at around 1 frame per second. This is because\CMF{ (1)} GamingAnywhere is
not optimized for the VR/networking architecture that
we used \CMF{with \OpenWVR{}}\CMFdel{in this paper.}\CMF{, and (2) }\CMFdel{
A few techniques customized network protocols)}\CMF{some of the customizations
that we used in \OpenWVR{} (such as modified network protocols)} cannot
work \CMFdel{with}in a cloud\CMF{-}computing environment. \CMFdel{Since }\CMF{Further, }GamingAnywhere
\CMF{can't use accelerated encoding and decoding because it }needs to accommodate
\CMFdel{the}\CMF{cloud-computing} abstractions\CMFdel{ of cloud computing, GamingAnywhere
misses the opportunity of accelerated encoding and decoding.}\CMF{, and its
FFmpeg-based encoding and decoding of H.264 video runs slowly}\CMFdel{
GamingAnywhere uses FFmpeg on both the
server and client to perform CPU-based encoding and decoding of H.264 video,
which is especially slow} on the Raspberry Pi. \OpenWVR{} \CMF{re}solves \CMFdel{the problems
that GamingAnywhere encounters}\CMF{these issues} by implementing GPU-based encoding and decoding
on both the host PC and MUD. While \OpenWVR{} still uses FFmpeg on the host PC
to facilitate GPU-based encoding, on the Raspberry Pi it calls the OpenMAX Bellagio
API directly to decode and render \CMFdel{the }H.264 frames.

\subsection{\CMFdel{Millimeter}\CMF{mm}Wave Wi\CMF{-}Fi}
\ignore{
The current \OpenWVR{} prototype uses IEEE 802.11ac as the link layer protocol.
The IEEE 802.11ac standard uses wireless bands around 5~GHz. With one antenna,
this standard can reach a theoretical bandwidth of 867 Mbit/s (i.e., 108 MiB/s).
Comparing the bandwidth for shipping raw 1080p images for both eyes at 60~GHz
(712~MiB/s) or raw 720p image at 60~GHz (316~MiB/s), IEEE 802.11ac still
falls short.  Therefore, the current \OpenWVR{} API compresses the generated
video content into H.264 format and decompresses the content in the \OpenWVR{}
MUD API to reduce the bandwidth demand.
}

Though recent advances in \CMFdel{millimeter wave}\CMF{mmWave} wireless technologies
(\CMFdel{e.g., }\CMF{like those specified by} IEEE
802.11ad) \CMFdel{claim}\CMF{are intended} to achieve \CMFdel{the}\CMF{a}
bandwidth of 7Gbit/s, \CMFdel{these}\CMF{such} technologies
suffer from serious constraints, including susceptibility to \CMFdel{blockage by objects in
between the source and the destination}\CMF{source-to-destination interference},
\CMFdel{very narrow angle of single beams}\CMF{restricted single-beam angles, }
\CMFdel{very short}\CMF{and limited} communication range\CMF{s}~\cite{MoVR}. In the early phases of developing
\OpenWVR{}, we \CMFdel{have done}\CMF{performed} quite a few field trials on
IEEE 802.11ad devices\CMFdel{.
However, the experiment can only achieve similar}\CMF{, but we only observed}
bandwidth\CMF{s similar to those of}\CMFdel{ as} IEEE 802.11ac
\CMFdel{in }wireless VR applications.


==> optimizations.tex <==
In addition, as
\OpenWVR{} only copies encoded data, this optimization reduces the latency
from memory copies by 6.7~ms, as
it avoids two significant data exchanges. Eliminating
redundant memory copies on the host does not help improve the latency on the
MUD, but this optimization still contributes a 37\% end-to-end latency reduction in \OpenWVR{}.
%This optimization requires the programmer to invoke \OpenWVR{} functions in the
%application. However, since this optimization reduces latency significantly,
%we do 
\subsubsection{Disable Buffering}
Since VR applications are very sensitive to latency, \OpenWVR{} cannot apply any
buffering mechanisms which multimedia streaming applications often use. 
Instead, \OpenWVR{} sends encoded H.264 frames to the network stack immediately. On the receiving end, \OpenWVR{} decodes and presents H.264 frames to the user as soon as they are fully received.
Disabling these video stream buffers makes \OpenWVR{} more sensitive to network jitters. 
However,
as the framework proposes the usage of a peer-to-peer network topology where each
sender-receiver pair uses their own dedicated channel,
network jitters rarely occurred across our experiments. 



different color spaces, \OpenWVR{} can leverage the underlying graphics cards' 
hardware-accelerated encoder to compress VR content using the native RGB format. 
On the Raspberry Pi-based MUD, the SoC also contains a hardware
accelerator supporting decoding RGB data, so \OpenWVR{} can completely avoid the overhead 
of converting color spaces. 

After applying this optimization, \OpenWVR{} can decrease the average encoding time
on the host machine from
10.3~ms to 5.6~ms, a 1.84\x{} speedup in video encoding.
On the MUD, latency from decoding H.264 format using RGB color space remains the same as the YUV
color space. As we maintain the same bitrate for encoded content, we do not
observe significant change in network latency. We also did not observe any
significant change in visual quality with transcoding avoidance. 
As a result, \OpenWVR{} reduces 
the total measured latency 
by about 4.7~ms, removing 26\% of the end-to-end latency from the baseline
implementation. 
%from 17.4 ms down to 13.3 ms.


\section{Optimizing \OpenWVR{}}
\label{sec:system}
%\label{sec:optimizations}
Using observations from the basic \OpenWVR{} implementation with
optimal parameters (Section~\ref{sec:breakdown}), \OpenWVR{} revisits 
and optimizes the system stacks to further reduce the end-to-end latency.
\OpenWVR{} proposes and integrates the following optimizations in various
layers of the system to address the delay in the basic implementation. 
\begin{itemize}
  \item {\bf Avoid transcoding.} \OpenWVR{} synchronizes the color spaces
that the GPU renders and video codec uses. This optimization can reduce the 
computational and memory overhead that changing color spaces incurs. 
  \item {\bf Eliminate GPU-main memory data movements.} \OpenWVR{}
reexamines the interactions between the GPU renderer and video codec. 
\OpenWVR{} eliminates unnecessary data movements between 
the GPU and system's main memory to reduce the delay due to ping-ponging VR
content on the host. 
  \item {\bf Direct network I/O.} \OpenWVR{} bypasses several layers in
the network stack to further avoid unnecessary memory copies and
computational overhead. 
  \item {\bf Feedback control.} \OpenWVR{} implements a custom feedback control
mechanism that allows the usage of larger GOP sizes to further reduce the
encoding latency and bandwidth demand. 
\end{itemize}

Table~\ref{table:latency} summarizes the effects of each optimization. These
optimizations help \OpenWVR{} eliminate 11.5~ms of latency, bringing the
average visual delay down to just about 1 60-FPS-frame. The following sections
will describe each optimization in detail. 

\subsection{Avoid transcoding}
With optimal parameters in the video codec, the largest contributor to latency is
converting the VR content the GPU generated as RGB into the YUV format. YUV format is generally the default for video compression applications because it allows efficient lossy compression that is difficult for humans to perceive.

Conversion between two different color spaces can require a considerable amount of 
overhead and add latency between the content generation and user
perception of the content. First, this requires additional memory space as well as memory access for 
the raw RGB content and the converted YUV format. Second, it consumes computing resources 
to perform the conversion. 
In conventional video streaming applications, the additional latency from
color space conversion and buffering is acceptable since these applications can tolerate
longer delays or do not require any user interaction with the content
generator. Therefore, these applications usually trade these additional
delays with higher video quality and lower bandwidth usage.

\ignore{
For example, using the YUV420 format can reduce the data size by 75\%. YUV that splits an image into its components of luma 
(black and white intensity) as well as 2D chrominance (color),
and then downsamples both chrominance components in the horizontal and vertical dimension, 
}
\ignore{
RGB data into YUV format and encoding that data in GPU. 
The default ffmpeg encoding library uses YUV color space, because using YUV
forms allows efficient lossy compression in ways that are difficult for humans to perceive. 
For example, our application uses YUV420, which splits an image into its components of luma 
(black and white intensity), and 2-dimensional chrominance (color), then downsamples both 
chrominance components in the horizontal and vertical dimension, reducing the data required 
for each by 75\%. 
}
%Our baseline program uses FFmpeg's swscale library to convert the RGBA data into the YUV 
%color space before sending it to the NVENC encoder. 
%For humans, this change is very difficult to perceive, but it reduces an image's size by 50\%.

As VR applications are extremely latency sensitive, \OpenWVR{} removes the process of converting color spaces. Avoiding transcoding between
different color spaces, \OpenWVR{} can leverage the underlying graphics cards' 
hardware-accelerated encoder to compress VR content using the native RGB format. 
On the Raspberry Pi-based MUD, the SoC also contains a hardware
accelerator supporting decoding RGB data, so \OpenWVR{} can completely avoid the overhead 
of converting color spaces. 

After applying this optimization, \OpenWVR{} can decrease the average encoding time
on the host machine from
10.3~ms to 5.6~ms, a 1.84\x{} speedup in video encoding.
On the MUD, latency from decoding H.264 format using RGB color space remains the same as the YUV
color space. As we maintain the same bitrate for encoded content, we do not
observe significant change in network latency. We also did not observe any
significant change in visual quality with transcoding avoidance. 
As a result, \OpenWVR{} reduces 
the total measured latency 
by about 4.7~ms, removing 26\% of the end-to-end latency from the baseline
implementation. 
%from 17.4 ms down to 13.3 ms.


\subsection{Eliminating redundant memory copies}
%
The initial implementation also reveals significant delays in memory
copies between the GPU device memory and system main memory. These memory
copies include the following. (1) Copying data from OpenGL pixel buffers 
from GPU memory into RAM for the FFmpeg library to convert RGB color space 
into YUV format; this is marked as Exchanging Pixel Data in Figure~\ref{fig:breakdown} and is measured as 4.8~ms. (2) FFmpeg needs to copy YUV formatted content back 
into the GPU device memory if the library relies on the GPU's hardware-accelerated encoder; this contributes to the measured latency of H.264 Encoding in Figure~\ref{fig:breakdown}. 
(3) \OpenWVR{} needs to copy data from the GPU device memory to the
network stack for the purpose of delivering the VR content to the MUD; this also contributes to the measured latency of H.264 Encoding in Figure~\ref{fig:breakdown}. 
With transcoding avoidance, \OpenWVR{} can potentially perform only the third
memory copy and remove the first two.

\ignore{
Though skipping the conversion from RGBA to YUV colorspace, the basic
\OpenWVR{} still copies pixel data from GPU memory into RAM, and from there back 
into GPU memory to be encoded. 
These data transfers can take several milliseconds, and are 
largely unnecessary if we copy the pixel data directly from the video-game-controlled GPU memory into FFmpeg-controlled 
GPU memory. 
We can take advantage of FFmpeg's integration with CUDA to reduce these two slow copies between GPU and CPU 
memory down to a single fast copy within GPU memory.}

To remove these redundant memory operations, \OpenWVR{} and the video
encoding library must work within the same process. Otherwise, the current
GPU runtime will still need to explicitly copy data from the GPU memory to
a shared memory location or use inter-process communication facilities, most 
likely the host DRAM for \OpenWVR{} and video codec library to access.
Therefore, we decided in our design of \OpenWVR{} to require the
application to invoke \OpenWVR{} API directly, instead of running a separate
daemon service on the host machine. Section~\ref{sec:API} describes
the software interface and demonstrates the moderate programming overhead.

Using the \OpenWVR{} API, the VR application can associate a GPU device
memory buffer with an \OpenWVR{} context, which is another thread running
concurrently with the VR application. Since the \OpenWVR{} context shares
the same memory space, including the GPU memory space, with the VR
application, \OpenWVR{} polls the GPU memory buffer periodically and invokes
the video encoding library on the GPU memory buffer directly. \OpenWVR{}
simply needs to move the final encoded VR content into the main memory, but
not any of the raw VR content that the GPU generates. 

This optimization eliminates all unnecessary memory copies. In addition, as
\OpenWVR{} only copies encoded data, this optimization reduces the latency
from memory copies by 6.7~ms, as
it avoids two significant data exchanges. Eliminating
redundant memory copies on the host does not help improve the latency on the
MUD, but this optimization still contributes a 37\% end-to-end latency reduction in \OpenWVR{}.
%This optimization requires the programmer to invoke \OpenWVR{} functions in the
%application. However, since this optimization reduces latency significantly,
%we do 

\subsection{Direct network I/O}
Our baseline program uses UDP (User Datagram Protocol) to communicate 
VR content and user input between devices, as is common among data streaming applications. UDP is
preferrable over TCP (Transmission Control Protocol), another popular network protocol, due to the latency sensitive characteristics of VR applications.
In addition, if an image frame is dropped, the application would rather skip it and render
the upcoming frame instead of waiting to receive the lost frame, making TCP's
reliability guarantee an unnecessary feature for VR applications. In
our \OpenWVR{}, the host communicates with peers using dedicated channels,
which lowers the probability of packet loss.

\ignore{
TCP would have been another option, since it is commonly used in networking, 
and it guarantees that all bytes sent by an application on one host will be received accurately and in order by an 
application on the other host. On an optimal physical network where no packets are lost, TCP's latency would approach 
that of UDP. But on the lossy wireless medium through which \OpenWVR{} is communicating, the lost data needs to be 
retransmitted until it is received correctly, which can greatly increase the latency of each video frame. In this manner, TCP could prevent the MUD from dropping video frames, but for the purposes of our live-streaming application, it is better to drop old and incomplete frames and wait for new ones than it is to receive frames late and present old data to the
user.}

While UDP is a good choice, it still
incurs some overhead to provide features that are unnecessary for \OpenWVR{}.
As an internetworking protocol, UDP expects packets to be sent through 
multiple routers, bridges, and other network-enabled machines on their way to reach their
destinations. To facilitate traveling along such a path, UDP attaches a header 
to every message, containing the length of the message, the port numbers of the 
source and destination, and a checksum which is used by the recipient to calculate 
whether any bytes were changed during transmission. In addition, UDP relies on
the layered network protocol stack, including the Internet Protocol to
decide the routing, the data link layer protocol (e.g., IEEE 802.11ac) for NIC-to-NIC communication, and the physical layer protocol for signal modulation. For
each layer of the network stack, the system needs to attach additional
headers and repartition the payload coming from another layer to different
sizes. Therefore, the conventional network stack also leads to additional
memory copies and buffering overhead. 
%, an IP header is additionally added which contains several fields to further identify the source and destination with IP addresses to allow for messages to be fragmented if necessary, and to prevent them from looping indefinitely through a network. The features and additional information provided by UDP and IP headers are unnecesary for \OpenWVR{}, where the MUD is expected to always be within range of the host PC's wireless transmitters, and therefore messages should not travel through any intermediary devices. \OpenWVR{} doesn't require a transport or network layer protocol at all, so we can improve performance by utilizing the data link layer.

%In \OpenWVR{} architecture, the system can avoid the overhead as the wireless network uses dedicated 
\OpenWVR{} proposes a direct network I/O mechanism to bypass these overheads by creating data link protocol packets
directly through the \OpenWVR{} kernel module.
As the \OpenWVR{} network architecture uses peer-to-peer connections so
that each pair of nodes communicates through their own dedicated channels,
\OpenWVR{} eliminates the demands of routing algorithms. Instead of using
the port number abstraction of UDP, \OpenWVR{} maps a transport layer buffer
from the kernel space directly to the application space through the kernel
module. The \OpenWVR{} API copies GPU data directly into the data link layer
buffer without going through any conventional routing and transport layer
protocols. We implement this customized protocol on both the host PC and
MUD. 

The direct network I/O mechanism allows \OpenWVR{} to reduce 3\% of network latency. Though direct network I/O only
contributes to a 1\% reduction in end-to-end latency, this mechanism lowers the
CPU overhead on processing network protocols. This is especially helpful to
reduce the energy consumption on battery-powered MUDs. 

\ignore{
for the \OpenWVR{} application over UDP. Using raw sockets allows hosts within range of 
each other to communicate in a peer-to-peer fashion even if they are connected to some 
intermediary device acting as an access point. Since the endpoints of raw communication 
are identified by their MAC addresses, and since \OpenWVR{}'s communications are unicast 
and do not include the access point's MAC address, the access point will ignore all such 
packets. The recipients each listen on the wireless medium for any packets addressed to 
their MAC address, regardless of the source address, so they will be able to process 
packets sent directly from each other. The MUD \OpenWVR{} application creates its raw 
socket with a parameter specifying for the operating system to only pass packets 
identified by the ethernet type "Local Experimental Ethertype," and the host PC sends 
packets with this ethertype. So long as the peers are connected on the same channel, 
they should be able to communicate directly in this manner. While such operation is 
possible, it is not preferred since there is a high chance that other devices are 
communicating with the access point on the same channel, causing interference and 
lowering the quality of service. It is also possible for a malicious device on the 
channel to perform a denial-of-service attack by broadcasting its own raw packets 
to the MUD's MAC address with the proper ethertype, although such an attack is 
possible for any sort wireless communication so long as proper address spoofing 
is used. For these reasons, it is still recommended that the devices establish a 
secure channel on which they are the only members.}
%Both Linux and Windows provide mechanisms for creating "raw sockets," which allow user applications to send data at the data link (Ethernet, 802.11, etc.) level. Sending via a raw socket allows us to send a custom ethernet frame, including the 14-byte header and up to around 1500 bytes of data, to a network interface. If being sent over a physical Ethernet link, then the frame is sent as-is, after a preamble is prepended and a checksum is appended to the message. In our case, where we send the frame over a wireless link, the operating system first converts the ethernet header to an 802.11 header and then broadcasts it. This allows us to bypass some processing involved in both the sending and receiving of data.

%For our baseline and improved trials, our endpoints are connected via a software-defined access point on the host PC, allowing the two devices to efficiently communicate directly with each other. In the \OpenWVR{} application, we found an increase in median network latency of 0.1 ms, although this only measures the transmission delay of the frames, which does not encompass the entire latency experienced in the network. To measure the difference in speed between UDP and raw, we created separate programs which use \OpenWVR{}'s UDP and RAW networking modules to send blank 100,000-byte frames to the MUD. We measured the round-trip time of the network as the time elapsed from the host PC application sending the first packet to the time that the host PC receives a UDP message from the end-user device confirming that the frame was received. We found that using UDP resulted in a round-trip time of 7.1 ms, while raw has a round-trip time of 6.9 ms. This 3\% speedup is statistically significant, although it doesn't significantly effect the user's perception of latency.

\subsection{Feedback control}
A reason that \OpenWVR{} chooses the current GOP size of 20 is because of the
trade-offs among latency, visual quality, and network bandwidth. With
protocols like UDP that provide no information to the sender about quality of service,
\OpenWVR{} can only use conservative GOP sizes.

In order to further decrease latency while decreasing the disruption of dropped 
frames and visual stuttering, we introduce an optimization in \OpenWVR{}'s
network protocol for the MUD to provide feedback to the host PC regarding dropped 
frames. Every time the MUD drops a frame 
due to not having received all of the data within a certain time frame, the
customized protocol sends a small message 
to the host PC that signals it to generate an I-frame on the next transmission. 
The MUD sends such a message after every frame received until it receives an I-frame. 
When the host fulfills an I-frame request, it will ignore 
further requests from the MUD for a certain period of time to prevent 
generation of consecutive large 
frames that will worsen network conditions. 

Using this feedback system allows \OpenWVR{} to increase the GOP size to
480. By resending a lost I-frame immediately, the MUD can still recover from 
dropped frames within 5 frames. Another problem with having a short GOP size is that I-frames take longer to encode, send and decode than P-frames, which causes a noticeable stutter whenever an I-frame is displayed to the user. With this new GOP size, the visual stutter occurs only once every 8 seconds, whereas at size 20 it occurs 3 times each second. This optimization slightly improves the
overall latency by 1\%, but the video quality is far superior.

%It also allows us to decrease the 
%target bandwidth to 20 Mbps, which decreases the network latency by about 0.5 ms, the 

\ignore{
 and it reduces our application's encoding time, from
average 4.5 ms down to 3.5 ms, while not significantly affecting the networking or decoding time. This makes 
for a further reduction of 5.7 ms, making the total latency 7.6 ms.}

\ignore{
By calling the \OpenWVR{} directly in the application, the \OpenWVR{} API
and the FFmpeg library act on behave of the application and will be able to 
share the GPU device memory without additional efforts. }

\ignore{
The \OpenWVR{} removes the redundant memory copies by initializing a CUDA 
context on the GPU and allocating GPU memory for RGB pixel data, returning a 
pointer to that memory. 
Then we minimally modify the VR application code to create an OpenGL pixel buffer
that will give us access to the pixel data currently being rendered to the screen. Then 
%We can register this buffer with Cuda using Cuda's OpenGL interoperability api, so that we will be able to map it as a
%CUDA pointer into GPU memory. Then we can call CUDA's memory copy function to copy the pixel data into the buffer 
%allocated by FFmpeg. 
%Reading pixels and copying data are synchronous functions and together they complete within 
%70~\us{}. 
}


%Though this optimization requires slight modification to application code, 


==> tableLatency.tex <==
\begin{table*}
\centering
%\scriptsize
\footnotesize
\begin{tabular}{|l|c|c|c|}
\hline
& Latency difference on & Latency difference on & Cumulative \\
Optimization 	  & Host PC (~\us{})       & MUD	(~\us{})    & difference\CMF{ }(~\us{}) \\
\hline
Plug-in modules & -4,710		& 0		    & -4,710\\
\hline
Intergration of video codec & -6,690		   & 0 & -11,400 \\
\hline
Direct network I/O & -292		& -119		   & -11,811\\
\hline
Feedback control  & -10		& -40		   & -11,851 \\
\hline
\hline
All optimizations  & -11,702		& -159		   & -11,851 \\
\hline
\end{tabular}
%\vspace{-2mm}
\caption{The improvement achieved by each cumulative \OpenWVR{} optimization\CMFdel{.}
\CMFcom{The first four values in the "Cumulative difference" column don't add up to the
total in the last row (-11,861), and the "Plug-in" row is the only row that appears to
yield the correct cumulative-difference values. In addition,
(1) ~\us{} are used in the table, but ms are used in the text---consider using only one unit for consistency, and
(2) the row label "Plug-in" doesn't seem to reflect the discussion of the API that appears in the text.}}
\label{table:latency}
\vspace{-0.1in}
\end{table*}
%& Latency difference on & Latency difference on & Cumulative \\
%Optimization 	  & Host PC (~\us{})       & EUD	(~\us{})    & difference(~\us{}) \\

